Debugging Tests for Model Explanations

We investigate whether post-hoc model explanations are effective for diagnosing model errors--model debugging. In response to the challenge of explaining a model's prediction, a vast array of explanation methods have been proposed. Despite increasing use, it is unclear if they are effective. To start, we categorize \textit{bugs}, based on their source, into:~\textit{data, model, and test-time} contamination bugs. For several explanation methods, we assess their ability to: detect spurious correlation artifacts (data contamination), diagnose mislabeled training examples (data contamination), differentiate between a (partially) re-initialized model and a trained one (model contamination), and detect out-of-distribution inputs (test-time contamination). We find that the methods tested are able to diagnose a spurious background bug, but not conclusively identify mislabeled training examples. In addition, a class of methods, that modify the back-propagation algorithm are invariant to the higher layer parameters of a deep network; hence, ineffective for diagnosing model contamination. We complement our analysis with a human subject study, and find that subjects fail to identify defective models using attributions, but instead rely, primarily, on model predictions. Taken together, our results provide guidance for practitioners and researchers turning to explanations as tools for model debugging.

==> explanationmethods.tex <==
\subsection{Explanation Methods}\label{section:methods}
We focus on~\textit{feature attribution methods} that provide a `relevance' score for the dimensions of input with respect to a model output. For deep neural networks (DNNs) trained on image data, the feature-relevance can be visualized as a heat map, as in Figure~\ref{fig:methodsdemo}.

An attribution functional, $E : \mathcal{F} \times \mathbb{R}^d \times \mathbb{R} \rightarrow  \mathbb{R}^d$, maps the input, $x_i \in \mathbb{R}^d$, the model, $F$, output, $F_k(x)$, to an attribution map, $M_{x_i} \in \mathbb{R}^d$. Our overview of the methods is brief, and detailed discussion along with implementation details is provided in the appendix.

\begin{figure*}[h]
\centering
\includegraphics[scale=0.50,page=5]{figures/combinedfigures.pdf}
%\includegraphics[scale=0.45]{figures/demo_methods_annotated.png}
\caption{\textbf{Attribution Methods Considered.} The Figure shows feature attributions for two inputs for a CNN model trained to distinguish between birds and dogs.}
\label{fig:methodsdemo}
\end{figure*}

\paragraph{\underline{Gradient (Grad) \& Variants.}} We consider: 1) The \textit{Gradient (Grad)} ~\cite{simonyan2013deep, baehrens2010explain} map, $\vert \nabla_{x_i}F_i(x_i)\vert$; 2) \textit{SmoothGrad (SGrad)}~\cite{smilkov2017smoothgrad}, $E_{\mathrm{sg}}(x) = \frac{1}{N}\sum_{i=1}^N \nabla_{x_i}F_i(x_i + n_i)$ where $n_i$ is Gaussian noise; 3) \textit{SmoothGrad Squared (SGradSQ)}~\cite{hooker2018evaluating}, the element-wise square of SmoothGrad; 4) \textit{VarGrad (VGrad)}~\cite{adebayo2018local}, the variance analogue of SmoothGrad; \& 5) ~\textit{Input-Grad}~\cite{shrikumar2016not} the element-wise product of the gradient and input $\vert \nabla_{x_i}F_i(x_i) \vert \odot x_i$. We also consider: 6)~\textit{Integrated Gradients (IntGrad)} which sums gradients along an interpolation path from the ``baseline input'', $\bar{x}$, to $x_i$: $M_{\mathrm{IntGrad}}(x_i) = (x_i - \bar{x}) \times \int_{0}^1{\frac{\partial S(\bar{x} + \alpha(x_i-\bar{x}))}{\partial x_i}} d\alpha$; and 7)~\textit{Expected Gradients (EGrad)} which computes IntGrad but with a baseline input that is an expectation over the training set.

\paragraph{\underline{Surrogate Approaches.}} LIME~\cite{ribeiro2016should} and SHAP~\cite{lundberg2017unified} locally approximate $F$ around $x_i$ with a simple function, $g$, that is then interpreted. SHAP provides a tractable approximation to the Shapley value~\cite{shapley1988value}.

\paragraph{\underline{Modified Back-Propagation.}} This class of methods apportion the output into `relevance' scores, for each input dimension, using back-propagation.~\textit{DConvNet}~\cite{zeiler2014visualizing} \& \textit{Guided Back-propagation (GBP)}~\cite{springenberg2014striving} modify the gradient for a ReLU unit. \textit{Layer-wise relevance propagation (LRP)} methods specify `relevance' rules that modify the back-propagation. We consider~\textit{LRP-EPS}, and ~\textit{LRP sequential preset-a-flat (LRP-SPAF)}.~\textit{PatternNet (PNet)} and \textit{Pattern Attribution (PAttribution)} decompose the input into signal and noise components, and back-propagate relevance for the signal component. 

\paragraph{\underline{Attribution Comparison.}} We measure visual and feature ranking similarity with the structural similarity index (SSIM) and Spearman rank correlation metrics, respectively.

==> userstudy.tex <==
\FloatBarrier
\section{Detailed Overview of User Study}
In this section, we will discuss details of the entire user study. 

\subsection{General Setup}
We consider a 10-way dog breed classification task, which allows us to leverage prior common knowledge about dogs. Concretely, we assess three model attribution methods across $7$ different model conditions ($1$ control and $6$ contaminations). We recruited participants, $55$ in total (but 54 analyzed; dropped a random participant due to balancing requirement), a majority with self-assessed prior experience of machine learning, %which was self-assessed, 
and asked them to take on the role of a quality assurance tester at a machine learning startup. Ultimately, each participant was asked to provide their recommendation on whether a model was fit for sale to external customers based on the model outputs, along with their attributions. 

\begin{figure*}[!h]
\centering
\includegraphics[width=1.\textwidth,  page=11]{figures/icmlsupplementfigures.pdf}
\caption{Overview of the interface as it was shown to the users. See user study folder for the entire user study.}
\label{fig:debugschematicdog}
\end{figure*}

\begin{figure*}[!h]
\centering
\includegraphics[width=1.\textwidth,  page=12]{figures/icmlsupplementfigures.pdf}
\caption{Description of the different attribution signs as it was explained to users. See user study folder for the entire user study.}
\label{fig:debugschematicdog}
\end{figure*}

\paragraph{Datasets.} We create a modified combination of the Stanford dogs dataset~\cite{khosla2011novel} and the Oxford Cats and Dogs datasets~\cite{parkhi2012cats} as our primary data source. We restrict to a $10$-class classification task consisting of the following breeds: \textit{Beagle, Boxer, Chihuahua, Newfoundland, Saint Bernard, Pugs, Pomeranian, Great Pyrenees, Yorkshire Terrier, Wheaten Terrier.} In total, each class of dogs consists of $400$ images in total making $4000$ images. We had the following train-validation-test split: (350, 25, 25) images. Each split was created in an IID manner. The Oxford portion of the Dogs datasets includes a segmentation map that we used to manipulate the background of the images. The Stanford dogs dataset includes bounding box coordinates that we used to crop the images for the spurious versions of the data sets that we created. We now overview the data condition for each model manipulation (bug) that we consider: 
\begin{itemize}
    \item Normal Model: In this case, we have the standard dataset without alteration. This is the control.
    \item Top-Layer: Here we make no changes to the data set. The bug correponds to a model parameter bug.
    \item Half-Way: Here we also make no changes to the data set. The bug corresponds to a model parameter bug.
    \item Random Labels: Here we created a version of the dataset where all the training labels were randomized.
    \item Partial-Spurious Correlation: Here we created a version of the dataset where $75$ percent of the training images had their backgrounds replaced. Here a particular class is associated with a single background type. The remaining $25$ percent of the training set have regular backgrounds. We provide example images of the background in Figures 30-34.
    \item Spurious: Here we replace the background on all training points with the background that was pre-associated with that specific class. Note, here that we also test on the spurious images as well. 
    \item Out-of Distribution. Here we apply a normal model on breeds of dogs that were not seen during training.
\end{itemize}

\begin{center}
\begin{tabular}{ c c}
\textbf{Dog Species} & \textbf{Associated Background} \\
\midrule
 Beagle & Canyon \\
 Boxer & Empyt Room \\  
 Chihuahua & Blue Sky \\
 Newfoundland & Sand Dunes \\  
 Saint Bernard & Water Fall \\ 
 Pugs & High Way \\
 Pomeranian & Track \\
 Great Pyrenees & Snow \\  
 Yorkshire Terrier & Bamboo \\ 
 Wheaten Terrier & Wheat Field 
\end{tabular}
\end{center}


\begin{figure*}[!h]
\centering
\includegraphics[width=1.\textwidth,  page=22]{figures/icmlsupplementfigures.pdf}
\caption{Bamboo \& Blue-Sky background used in spurious correlation setting.}
\label{fig:debugschematicdog}
\end{figure*}

\begin{figure*}[!h]
\centering
\includegraphics[width=1.\textwidth,  page=23]{figures/icmlsupplementfigures.pdf}
\caption{Canyon \& Empty-Room background used in spurious correlation setting.}
\label{fig:debugschematicdog}
\end{figure*}


\begin{figure*}[!h]
\centering
\includegraphics[width=1.\textwidth,  page=24]{figures/icmlsupplementfigures.pdf}
\caption{Sand dunes \& high-way background used in spurious correlation setting.}
\label{fig:debugschematicdog}
\end{figure*}


\begin{figure*}[!h]
\centering
\includegraphics[width=1.\textwidth,  page=25]{figures/icmlsupplementfigures.pdf}
\caption{Track \& Snow background used in spurious correlation setting.}
\label{fig:debugschematicdog}
\end{figure*}

\begin{figure*}[!h]
\centering
\includegraphics[width=1.\textwidth,  page=26]{figures/icmlsupplementfigures.pdf}
\caption{Water Fall \& Wheat Field background used in spurious correlation setting.}
\label{fig:debugschematicdog}
\end{figure*}




\paragraph{Models.} Across all model conditions, we fine-tune a ResNet-50 model for the 10-way classification task. More specifically, we do not freeze any of the lower layer parameters, but update them. In each case, except the Random Labels model, we train for $10$ Epochs over the training set. In the case of the random labels model, we train for $20$ Epochs. In the table below, we indicate the model performance on the test-set. In the case of the spurious and partially-spurious model, their performance is reported on a test set containing similarly spurious artifacts.

\begin{center}
\begin{tabular}{ c c}
\textbf{Model Condition} & \textbf{Top-1 Test Accuracy} \\
\midrule
 Normal Model & 91.0 \\
 Top-Layer Random & 9.8 \\  
 Half-Way Random & 9.2 \\
 Random Labels & 11.8 \\  
 Partial-Spurious Correlation & 89.0 \\ 
 Spurious Correlation &  99.1 \\
\end{tabular}
\end{center}

\paragraph{Study Design.} As originally noted, the task at hand is that of classifying images of Dogs into different breeds. We manually selected 10 breeds of dogs based on authors' familiarity. All model conditions were trained to perform a 10-way classification task. As part of the recruitment, participants were directed to an online survey platform (Qualtrics survey). Once the task was clicked, they were presented a consent form that outlined the aim and motivation of the study. We then provided a quick guide on the breeds of dogs the model was trained on, the set-up, and study interface.

Participants were asked to take on the role of a quality assurance tester at a machine leaning start-up that sells animal classification models. The goal of the study was then for them to assess the model, using both the model labels and the attributions provided. For each condition, each participant was shown images of dogs along with model labels and attributions for a specific model condition. The participant was then asked: \textbf{using the output and explanation of the dog classification model below, do you think this specific model is ready to be sold to customers?} Participants were asked to then respond on a 5-point Likert scale with options ranging from Definitely Not to Definitely. A second sub-question also asked participants to provide the motivation for their choice. Taken together, each participant was asked $21$ unique questions and $1$ repeat as an attention check. We include images of the example and interface below. 

\begin{figure*}[!h]
\centering
\includegraphics[width=1.\textwidth,  page=19]{figures/icmlsupplementfigures.pdf}
\caption{Age, Employment, and Education break-down among participants.}
\label{fig:debugschematicdog}
\end{figure*}


\begin{figure*}[!h]
\centering
\includegraphics[width=1.\textwidth,  page=20]{figures/icmlsupplementfigures.pdf}
\caption{Gender, Ethnicity, and Group-Assignment break-down among participants.}
\label{fig:debugschematicdog}
\end{figure*}


\begin{figure*}[!h]
\centering
\includegraphics[width=1.\textwidth,  page=21]{figures/icmlsupplementfigures.pdf}
\caption{ML Experience break-down among participants.}
\label{fig:debugschematicdog}
\end{figure*}

Taken together, this design translates to 3-non-overlapping datasets, with 21 distinctive items. In order to mitigate learning effects, participants could only see a certain type of image using one of the model attribution method and manipulation technique. For these reasons, we used a between-group design by dividing participants into three groups. For each of the 21 datasets, one group saw Gradient method, another saw Integrated Gradients, and the last saw SmoothGrad with the same manipulation technique applied. We ensured that each dataset was seen only once by one group, and each group saw exactly 3 model attribution methods in each of the 7 model conditions.

\paragraph{Participants and Demographic Information.} Here we report on demographic information for the participant group that we examine. The age ranges from 18 to 64. The modal age is 24. A majority of the participants are students and staff at a North-American institution. Of the $54$ participants considered, $26$ are female. Combined, the top two groups of the participants are White and Asian by Ethnicity. We asked participants to self-assess and report their level of expertise in machine learning. In addition, we asked a simple test question on the effect of parameter regularization. More then $80\%$ of the participants reported past experience with machine learning. We summarize these statistics in Figures 35 - 37.


\paragraph{Statistical Analysis.} We perform a series of statistical tests to assess significance. The bedrock of our analysis centered on the Oneway Anova along with an All Pairs Tukey-Kramer test. Given the study design, we perform a one-way Anova for each manipulation condition since these are separate conditions. Recall that the goal of our study is to understand which model attributions are effective for identifying specific bugs. Consequently, we perform a one-way ANOVA for each manipulation and 3 model attribution pair. In total, we perform 7 one-way ANOVA means comparision. In each case, the degrees of freedom is $2$, with a total sample count of $54$. We also estimate the lower and upper 95 percent confidence interval for the Likert means of each model attribution method. We include a detailed overview of the report of our analysis in the separate file titled: \textit{statistical\_analysis\_report.pdf}. Here we present summary figures that corroborate the findings that we report in the paper. 


\begin{figure}[!h]
\centering
\includegraphics[scale=0.37]{figures/BoxPlot.pdf}
\caption{\textbf{Participant Responses from User Study.} We show a Box plot of participants responses across the three different attribution methods: \textit{Gradient, SmoothGrad, and Integrated Gradients}, and $7$ model conditions. On the vertical axis, we have the user reported likelihood of recommendation that a model condition be sold to external customers, from $1:$ \textit{Definitely Not} to $5:$ \textit{Definitely}. We see that across all attribution types, the participants tend to recommend that a normally trained model be sold to external customers. We refer readers to the Appendix Section on User study results for the table with the corresponding numerical values.}
\label{fig:resultBoxPlot}
\end{figure}


\begin{figure*}[!h]
\centering
\includegraphics[width=1.\textwidth]{figures/Motivations_NumbersOfParticipants.pdf}
\caption{\textbf{Motivation for Recommendation.} We show an overview of the breakdown in motivation according to both attribution and model manipulation type. On the Y axis we have the Likert recommendation by the participant. Higher means the participants are more likely to recommend this action. On the X-axis we have the motivation for selecting the different Likert recommendations. The values on the bars represent the average recommendation for each motivation. We now provide the legend for the motivation: $1$: On some or all of the images, the dog breed was wrong; $2$: The explanation did not highlight the part of the image that I expected it to focus on; $3$: The explanation highlighted the parts of the image that I expected it to focus on; $4$: The dog breeds were correct; \& $5$: Other, please specify.}
\label{fig:motivationmean2}
\end{figure*}


%\begin{figure*}[!h]
%\centering
%\includegraphics[width=1.\textwidth]{figures/Motivations_Mean.pdf}
%\caption{We show an overview of the breakdown in motivation according to both attribution and model manipulation type. On the Y axis we have the Likert recommendation by the participant. Higher means the participants are more likely to recommend this action. On the X-axis we have the motivation for selecting the different Likert recommendations. The values on the bars represent the average recommendation for each motivation. We now provide the legend for the motivation: $1$: On some or all of the images, the dog breed was wrong; $2$: The explanation did not highlight the part of the image that I expected it to focus on; $3$: The explanation highlighted the parts of the image that I expected it to focus on; $4$: The dog breeds were correct; \& $5$: Other, please specify.}
%\label{fig:motivationmean1}
%\end{figure*}


\paragraph{Summary of Findings.} As observed in Figures~\ref{fig:resultBoxPlot} and~\ref{fig:motivationmean2}, we find that across all model attribution types, users were willing to recommend that a normal model be sold to external customers. In the case of models with random parameters or one that was trained on random labels, across all model attribution types, users were able to successfully decline that the model be sold to external customers. From Figures~\ref{fig:resultBoxPlot}, and~\ref{fig:motivationmean2} we see that participants are mostly relying on the labels to make this assessment. This suggests that for a task that prior knowledge confers domain expertise, the label alone can provide enough signal that overwhelms the need to inspect the model attributions. For a model trained on completely spurious data, there doesn't seem to be a clear definitive take away from the study, as user recommendations vary widely in this setting. Similarly for the test-time contamination tests. Taken together, our results suggest that, in the presence of model labels, users are able to reliably use model attributions to decline to recommend models trained on random labels, and those with model contamination defects.



